A Truly Joint Neural Architecture for Segmentation and Parsing

Contemporary multilingual dependency parsers can parse a diverse set of languages, but for Morphologically Rich Languages (MRLs), performance is attested to be lower than other languages. The key challenge is that, due to high morphological complexity and ambiguity of the space-delimited input tokens, the linguistic units that act as nodes in the tree are not known in advance. Pre-neural dependency parsers for MRLs subscribed to the joint morpho-syntactic hypothesis, stating that morphological segmentation and syntactic parsing should be solved jointly, rather than as a pipeline where segmentation precedes parsing. However, neural state-of-the-art parsers to date use a strict pipeline. In this paper we introduce a joint neural architecture where a lattice-based representation preserving all morphological ambiguity of the input is provided to an arc-factored model, which then solves the morphological segmentation and syntactic parsing tasks at once. Our experiments on Hebrew, a rich and highly ambiguous MRL, demonstrate state-of-the-art performance on parsing, tagging and segmentation of the Hebrew section of UD, using a single model. This proposed architecture is LLM-based and language agnostic, providing a solid foundation for MRLs to obtain further performance improvements and bridge the gap with other languages.

==> error_analysis.tex <==
\paragraph{Error Analysis}
% [TODO - this section is repetitive, with some internal inconsistencies, and very long. can you put the results of the categories in a table and make the text non repetitive and shorter?]
To gain insights into the practical implementation of our model for downstream tasks, we performed an error analysis on a subset of 50 sentences from the Hebrew UD dev set. Based on our analysis, a total of 108 errors were identified, classified into four distinct categories: prediction errors, gold errors, ambiguous errors, and others (see Table \ref{table:error types}). In the case of ambiguous errors, we observed instances of uncertainty between the predicted annotation and the gold standard, or with other optional analyses.
In addition to the aforementioned categorization, in table \ref{table:label errors} we further categorized the errors based on labels. The predominant error type is associated with the PP attachment issue, where 20\% of the errors involve the obl and nmod relations, which indicate the complements of the verb and the noun, respectively. For example, in the sentence \textit{mby'ym `wbdym zrym l y/sr'l}, the head of the phrase \textit{l y/sr'l} ("to Israel") is identified as the noun \textit{`wbdym zrym} ("foreign workers") using the nmod label, instead of being linked to the verb \textit{mby'ym} ("bring") with obl label. 
% Similarly, in the sentence \textit{kl y/sr'ly h mnwsh b qrb lylh b /s.t.h bnwy ywd`} ("every Israeli experienced in a night battle in a built-up area knows"), the modifier \textit{qrb} ("battle") is erroneously connected to the verb \textit{mnwsh} ("experienced") with the obl label, instead of being associated with the noun \textit{/s.t.h} ("area") using the nmod label. 
Another prevalent error arises with the conj label, which designates the connection between two elements joined by a coordinating conjunction. This relationship holds significance in comprehending how different components within a sentence are interrelated, particularly in complex sentence structures. 
% The majority of errors in this category are attributed to head errors, where the label "conj" is correctly assigned, but the head is inaccurately identified. 
For instance, in the sentence \textit{h/syrwt pw`l l.sm.swM msprM /sl h`wbdyM hzryM wlhknst `wlyM .hd/syM bmqwmM} ("The service works to reduce the number of foreign workers and bring in new immigrants in their place") the segment \textit{hknst} ("bring") should be connected to \textit{.sm.swM} ("reduce") due to the coordinating conjunction "and", but it is erroneously linked to \textit{.sm.swM} ("h`wbdyM").

In addition to addressing syntactic errors, our analysis also covers segmentation errors. Among the errors identified, there were 8 instances of segmentation errors, with 5 of them involving missing or redundant determiners. These errors are generally considered minor in nature.


